Partial Typing for Asynchronous Multiparty Sessions

Formal verification methods for concurrent systems cannot always be scaled-down or tailored in order to be applied on specific subsystems. We address such an issue in a MultiParty Session Types setting by devising a partial type assignment system for multiparty sessions (i.e. sets of concurrent participants) with asynchronous communications. Sessions are possibly typed by "asynchronous global types" describing the overall behaviour of specific subsets of participants only (from which the word "partial"). Typability is proven to ensure that sessions enjoy the partial versions of the well-known properties of lock- and orphan-message-freedom.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{S. Alves and I. Mackie (Eds.): 13th International Workshop\\
on Developments in Computational Models 2023 (DCM'23).\\
EPTCS 408, 2024, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.408.1}{10.4204/EPTCS.408.1}}
\pdfoutput=1

